DocQT: Improving Document Forgery Localization Robustness via Diverse JPEG Quantization Tables

Document manipulation localization models achieve strong performance on public benchmarks yet fail to generalize to operational document workflows. We identify a critical and overlooked source of this gap: the mismatch between the narrow distribution of JPEG quantization tables used during training -restricted to standard libjpeg quality factors -and the heterogeneous compression profiles encountered in real-world insurance document pipelines. To isolate this factor, we conduct a controlled factorial study comparing two architectures with contrasting levels of quantization table awareness -FFDN [2] and Mesorch [20] -each trained under either standard quality factor augmentation (Standard-QT ) or operationally calibrated quantization tables sampled from DocQT, a quantization-table bank derived from a MAIF operational image corpus (Real-QT ), and evaluated under three recompression conditions. Training under Real-QT yields substantial localization gains on DocTamper [15] and significantly reduces the pixel-level false positive rate on authentic operational documents, but only for architectures that explicitly ingest the quantization table as input. The released DocQT quantization-table dataset and compression-reproduction material are directly available at https://github.com/Kyliroco/Improving-Document-Forgery-Localization-Robustness-via-Diverse-JPEG-Quantization-Tables. These results demonstrate that standard quality factor augmentation does not adequately proxy operational compression diversity, and that architectural choices explicitly conditioning on the quantization table provide a meaningful robustness advantage for real-world deployment.

==> sections/methode.tex <==
\section{Methodology}
\label{sec:methodology}
\subsection{Experimental Framework and Model Selection}
All experiments are conducted within the ForensicHub framework~\cite{du_forensichub_2025}, which provides a unified training and evaluation infrastructure across forensic tasks and natively implements both FFDN~\cite{chen_enhancing_2025} and Mesorch~\cite{zhu_mesoscopic_2024}. Among the models available in ForensicHub, these two are selected because they represent opposite ends of a structural spectrum directly relevant to the central question of this paper: FFDN explicitly ingests the JPEG quantization table as an input, making it by design sensitive to quantization table distribution shift, whereas Mesorch relies exclusively on implicit pixel-domain and DCT-domain artifacts without any explicit quantization table processing. The remaining models integrated in ForensicHub --- such as ManTra-Net~\cite{wu_mantra-net_2019}, CAT-Net~\cite{kwon_learning_2022}, or PSCC-Net~\cite{liu_pscc-net_2022} --- do not exhibit this structural contrast with respect to quantization table awareness, and their inclusion would not add discriminative information for the specific hypothesis under investigation.
FFDN~\cite{chen_enhancing_2025} and Mesorch~\cite{zhu_mesoscopic_2024} are selected because they represent opposite ends of a structural spectrum directly relevant to the central question of this paper. As described in Section~\ref{sec:doc_localization}, FFDN inherits from DTD~\cite{qu_towards_2023} a Frequency Perception Head that ingests the quantization table as an explicit input, making it by design sensitive to quantization table distribution shift. Mesorch, as described in Section~\ref{sec:natural_localization}, does not exploit the quantization table explicitly, which makes it a particularly informative counterpoint for assessing the role of quantization table awareness under distribution shift.
% \subsection{Experimental Framework} 

% All experiments are conducted within the ForensicHub framework~\cite{du_forensichub_2025}, which provides a unified training and evaluation infrastructure across forensic tasks. ForensicHub natively integrates DocTamper, T-SROIE, and RTM on the document side, and supports Mesorch as an IMDL model. FFDN, being a more recent document-oriented method, is integrated manually following the same protocol. The two models evaluated in this study are FFDN~\cite{chen_enhancing_2025}, a document-specialized architecture combining visual and frequency branches, and Mesorch~\cite{zhu_mesoscopic_2024}, an IML model designed to capture artifacts at the mesoscopic level by integrating both microscopic low-level traces and macroscopic object-level semantics through parallel CNN and Transformer branches. Comparing these two models allows us to contrast a method designed specifically for document images against one conceived for natural image manipulation localization. 

% % Transition vers la section suivante à placer

% \subsection{Proposed Approach}

% We dediced to select two models of the ForensicHub: they provide complementary approaches to manipulation localization~\cite{du_forensichub_2025}. FFDN~\cite{chen_enhancing_2025} is a document-specialized architecture that addresses the challenge of subtle tampering by jointly modeling the spatial and frequency domains. It builds on a ConvNeXt~V2 backbone and introduces a Visual Enhancement Module~(VEM), which injects frequency-domain information into the RGB feature space using zero-initialized convolutions, and a Wavelet-like Frequency Enhancement~(WFE) module, which explicitly decomposes features into high- and low-frequency components to retain fine-grained tampering traces that standard downsampling discards. Crucially, the model ingests DCT coefficients and the JPEG quantization table as explicit inputs via the Frequency Perception Head~(FPH)~\cite{qu_towards_2023}, making it directly sensitive to the quantization table distribution of its training data~\cite{kwon_learning_2022}. 

% Mesorch~\cite{zhu_mesoscopic_2024} adopts a fundamentally different perspective motivated by the observation that manipulation operates simultaneously at the microscopic level through low-level forensic traces and at the macroscopic level through semantic object-level alterations. To capture both, Mesorch runs a CNN branch and a Transformer branch in parallel: the CNN processes high-frequency DCT-enhanced features to capture local textural anomalies, while the Transformer processes low-frequency DCT-enhanced features to model global semantic context. An adaptive weighting module then dynamically adjusts the contribution of each scale before producing the final mask. By design, Mesorch does not exploit the quantization table explicitly~\cite{zhu_mesoscopic_2024}, which makes it a particularly informative counterpoint to FFDN for assessing the role of quantization table awareness under distribution shift. 

% \begin{figure}[ht] 
%     \centering 
%     \includegraphics[width=\linewidth]{images/FFDN.png} 
%     \caption{Architecture of FFDN~\cite{chen_enhancing_2025}. CA: Channel Attention; SA: Spatial Attention; E1--E4: ConvNeXtV2 encoder stages; F1--F4: feature maps at the corresponding scales.} 
%     \label{fig:ffdn} 
% \end{figure} 
% \begin{figure}[ht] 
%     \centering \includegraphics[width=\linewidth]{images/mesorch.png} 
%     \caption{Architecture of Mesorch~\cite{zhu_mesoscopic_2024}. The high-frequency enhanced image is processed by the LocalFeatureEncoder (CNN branch) while the low-frequency enhanced image is processed by the GlobalFeatureEncoder (Transformer branch). An adaptive weighting module fuses predictions across scales.} 
%     \label{fig:mesorch} 
% \end{figure} 

% \subsection{Evaluation Criteria} 
% \label{sec:evaluation} All models in this study produce a pixel-level probability map $P \in [0,1]^{H \times W}$, from which a binary prediction mask $\hat{M}$ is derived by thresholding at $\tau = 0.5$: 

% \begin{equation} 
%     \hat{M}(i,j) = \mathbb{I}\bigl(P(i,j) \geq \tau\bigr). 
% \end{equation} 

% Given the ground-truth binary mask $M_{gt}$ provided by each dataset, the following pixel-level quantities are defined: 

% \begin{align} 
%     TP_{\text{pix}} &= \textstyle\sum_{i,j} \mathbb{I}\bigl(\hat{M}(i,j)=1 \wedge M_{gt}(i,j)=1\bigr), \\ FP_{\text{pix}} &= \textstyle\sum_{i,j} \mathbb{I}\bigl(\hat{M}(i,j)=1 \wedge M_{gt}(i,j)=0\bigr), \\ FN_{\text{pix}} &= \textstyle\sum_{i,j} \mathbb{I}\bigl(\hat{M}(i,j)=0 \wedge M_{gt}(i,j)=1\bigr). 
% \end{align} 

% \subsubsection{Localization on Tampered Images}

% On images that contain at least one altered pixel (i.e., $\sum_{i,j} M_{gt}(i,j) \geq 1$), localization performance is measured by the \textbf{Intersection over Union}~(IoU) and the pixel-level \textbf{F1 score}~\cite{ma_imdl-benco_2024,du_forensichub_2025}: \begin{equation} \mathrm{IoU} = \frac{TP_{\text{pix}}}{TP_{\text{pix}} + FP_{\text{pix}} + FN_{\text{pix}}}, \end{equation} 

% \begin{equation} 
%     F_1^{\text{pix}} = \frac{2\,TP_{\text{pix}}}{2\,TP_{\text{pix}} + FP_{\text{pix}} + FN_{\text{pix}}}. 
% \end{equation} 
% Both metrics are computed per image and averaged across the evaluation set. 

% \subsubsection{Spurious Activation on Unaltered Images} Several datasets in this study contain exclusively unaltered images (SROIE, FUNSD, and the [ANONYMIZED ORGANIZATION] operational set) and are included specifically to measure the tendency of models to produce spurious activations~\cite{guillaro_trufor_2023}. For any unaltered image, the ground-truth mask is evenly zero ($M_{gt} = \mathbf{0}$), so every predicted positive pixel is by definition a false positive. The \textbf{pixel-level false positive rate} $\mathrm{FPR}  _{\text{pix}}$ equation \eqref{fpr_pix} is therefore defined as the fraction of pixels incorrectly predicted as altered: 

% \begin{equation} 
%     \mathrm{FPR}_{\text{pix}} = \frac{FP_{\text{pix}}}{H \times W}, \label{fpr_pix} 
% \end{equation}

% where $H \times W$ is the total number of pixels in the image. This quantity is computed per image and reported as a mean value across the reference set, the latter being more sensitive to pathological cases where a model produces a large contiguous activation on an intact image~\cite{guillaro_trufor_2023}. A low $\mathrm{FPR}_{\text{pix}}$ on unaltered images combined with a high $F_1^{\text{pix}}$ on tampered images constitutes the primary criterion for assessing robustness to quantization table distribution shift, which is the central experimental question of this study.
